Measuring Corporate Digital Divide with web scraping: Evidence from Italy

With the increasing pervasiveness of ICTs in the fabric of economic activities, the corporate digital divide has emerged as a new crucial topic to evaluate the IT competencies and the digital gap between firms and territories. Given the scarcity of available granular data to measure the phenomenon, most studies have used survey data. To bridge the empirical gap, we scrape the website homepage of 182 705 Italian firms, extracting ten features related to their digital footprint characteristics to develop a new corporate digital assessment index. Our results highlight a significant digital divide across dimensions, sectors and geographical locations of Italian firms, opening up new perspectives on monitoring and near-real-time data-driven analysis.

==> findigs.tex <==
\section[sec:findings]{Clustering}

In this section, we show the results of our first analysis considering only the web-related features.
As we can notice from the explorative analysis of the web-related features (see Section \ref{subsec:web}), the different features present evident territorial patterns, at least at province level.
Therefore, taking into account that the enterprise aggragated behaviour on the web is similar in areas that are spatially close, we can leverage these several similarities to determine clusters of territories (e.g. provinces and municipalities) that show similar patterns.

In this analytical step, we take into account only the web-related features computed by means of our crawler. These features intend to describe the internal quality of the web-site and the ones the are more related to the interaction with an external user such as social media profiles, loading speed, etc. 

Thus, for each firm included in our dataset, with a reachable web-site, we extracted a set of features, we perform a normalization step with a $MinMax$ scaler, then we aggregate these variables at the required spatial granularity level (i.e. province or municipality) computing the average, or the percentage on the total of enterprises included in our dataset.
Once the dataset is ready, we performed a $k-means$ clustering, where the data points in input are all provinces, or all the municipalities with the relative feature vector.
The clustering results at province level are shown in Figure~\ref{fig:clusteringprovince} where we set the number $k$ of clusters equal to 3\footnote{we computed the best number of clusters through the classical elbow method. We omitted here the graph to focus on more useful insights.}.
From the figure, it is easy to highlight the fact that the procedure detects 3 macro areas: North, Center and South, completely in a \textit{data-driven} manner: it is able to find the Three Italies. Notice that the geographical information is not included in the feature vector.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/clustering_provinciale.png}
    \caption{Clustering performed at province (NUTS3) level.}
    \label{fig:clusteringprovince}
\end{figure}

\todo{aggiungere il plot dei centroidi e aggiungere un commento}

The results of the clustering applied at municipality level are reported in Figure~\ref{fig:clusteringmun}. In this analysis, we consider only the municipalities with at least 10 enteprises. Also in this case, we applied the $k-means$ algorithm with $k$ equal to 3. 
Also in this case, the three cluster present a different spatial spread. The cluster represented in red is more concentrated in highly developed territory and big cities. 
The cluster in green is more in areas that are in more suburbs areas. The cluster in blue, instead, in located in marginal areas are mainly in the South. 

In both cases, the clustering results show clear patterns, dividing the national territory between more and less known developed areas.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/clustering_comunale.png}
    \caption{Clustering performed at municipality level.}
    \label{fig:clusteringmun}
\end{figure}


==> methodology.tex <==
\section{Methodology}\label{sec:methodology}

This section describes the adopted methodology we adopt for the empirical analysis of the corporate Digital Divide. We rely on 182,705 firms out of the initial sample (composed of 347,010 firms), because a consistent number of firms showed null values for employment, a useful indicator to categorise the size of each firm in different groups. We employ an OLS regression with the following specification is the following:
\begin{equation*}
    y = \alpha + \beta_lx_l + \beta_cx_c + \epsilon
\end{equation*}
where $y$ represents the 10 Digital Dimensions, $x_l$ is the vector that represents the relevant characteristics of the firm, namely age, location (in terms of urban context and regions), sector, size. We control for the possible impact of wide band, represented by vector $x_c$ . 
% \end{equation*}


Figure \ref{fig:methodology} shows the workflow to compute and validate WAI of Italian firms. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.3\columnwidth]{figures/todo_paper_digital_divide.png}
    \caption{Methodology flow}
    \label{fig:methodology}
\end{figure}

==> old_tex/clustering.tex <==
\section[sec:results]{Spatial clustering of corporate website features}\label{sec:clustering}
As we can notice from the explorative analysis of the previous section (see Section \ref{sec:data}), some of the features present evident territorial patterns, at least at NUTS-3 level.
Therefore, taking into account the hypothesis that the aggregated behaviour of firms on the web is similar in spatially close areas \citep{Forman2005, Schleife2010, Blanketal2018}, we can leverage this property to determine if clusters of territories (e.g. NUTS-3 regions and municipalities) show a similar pattern.

In this analytical step, we take into account only the web-related features computed by means of our crawler. Thus, for each firm included in our dataset, with a reachable website, we extracted eleven features, inverting the scale of the values (from low quality to high quality) where necessary (the length of the URL, Facebook, request time, security header) for the purpose of interpretability.
After we perform a normalisation step with a $MinMax$ scaler, aggregating the abovementioned variables at the NUTS-3 and municipality level, computing the average for all the features except for the ones related to social media.
For these, we consider the percentage of enterprises adopting a specific social media over the total of enterprises included in our dataset.
THen, we applied the $k-means$ clustering taking in input the aggregated features at NUTS-3 regions, and subsequently the same set of features aggreated at municipality level.
The clustering results at NUTS-3 level are shown in the map on the left of Figure~\ref{fig:clustering:provinciale}. Where we set the $k$ number of clusters equal to 3\footnote{we computed the optimal number of clusters through the classical and well known elbow method.}. 

From the map, it is easy to highlight the fact that the procedure detects three macro-regions: North, Center and South, in a completely \textit{data-driven} manner (notice that the geographical information is not included in the feature vector).

Figure \ref{fig:clustering:provinciale} reports on the left the centroids of the three identified clusters, showing how the groups behave across the examined features. 
The colours are shared between the two figures. Thus, the centroids of the yellow cluster are drawn with a yellow line and so on.
Concerning the centroids, the northern regions (in yellow) display marked higher average performance for links, website age and LinkedIn, security, access time and length url. Centre and southern regions show similar trends in 6 features, while a different behaviour emerges on security, access time, length url, Facebook and Instagram.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \toprule
    \includegraphics[width=0.48\columnwidth]{figures/clustering_provinciale.png} &
    \includegraphics[width=0.48\columnwidth]{figures/centroids_clustering_provinciale.png} \\
    \bottomrule
    \end{tabular}
    \caption{Clustering results at NUTS3 level. On the left the spatial distribution of the clusters. NUTS-3 depicted with the same color indicates that they belong to the same cluster. On the right the relative centroids of the three identified clusters. The colours of the lines correspond to the ones in the map.}
    \label{fig:clustering:provinciale}
\end{figure}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/clustering_provinciale.png}
%     \caption{Clustering performed at province (NUTS3) level.}
%     \label{fig:clusteringprovince}
% \end{figure}

% \todo{aggiungere il plot dei centroidi e aggiungere un commento, una parte può essere tradotta da pezzo sotto in italiano}

% \fabio{Analizzando i centroidi dei cluster individuati possiamo vedere come le tre macro aree rappresentino comportamenti medi abbastanza differenti. 
% Il cluster localizzato maggiormente nell’area dell’Italia del Nord ha – generalmente – caratteristiche che indicano una maggiore qualità del sito, una più alta velocità di caricamento e un maggior orientamento sui social con target professionale. 
% Il cluster che comprende prevalentemente le province del centro Italia, non si discostano molto dalle caratteristiche del cluster del Nord Italia, ma hanno alcune differenze sulla presenza nei social. 
% Il cluster localizzato soprattutto nel Sud d'Italia, ha un comportamento medio abbastanza differente rispetto agli altri due, sia in termini di qualità del sito che di facilità di engagement verso l’esterno. In media le province di questo cluster hanno tempi di caricamento più lenti, e un molta più presenza su Facebook rispetto a Linkedin.}

The results of the clustering applied at municipality level are reported in Figure~\ref{fig:clustering:comunale}. In this analysis, we consider only the municipalities with at least 10 enteprises to avoid that small groups high/low performant firms could provide misleading interpreation. Also in this case, we applied the $k$-means algorithm with $k$ equal to 3. 
Even in this case, we can highlight 3 ``distinct'' behaviours, even if with less marked differences (see the centroid plot on the right of Figure~\ref{fig:clustering:comunale}).

 The blue cluster in Figure~\ref{fig:clustering:comunale} comprehends developed areas such as big cities like Milan and Genova, industrial cities in the north-east (Venezia, Padova, Verona) and Emilia Romagna (e.g. Bologna, Modena, Parma, Ferrara), regional capitals of Trentino Alto Adige (Trento and Bolzano) and cities located in Tuscany (such as Firenze and Pisa). The red cluster prevalently shows the profile of cities located in the nearby of the abovementioned urban poles.
Finally, the cluster in green display mainly coastal cities in the centre and south regions of the countries, with important cities like Rome, Naples, Bari, Cagliari and Palermo.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \toprule
    \includegraphics[width=0.48\columnwidth]{figures/clustering_comunale.png} & \includegraphics[width=0.48\columnwidth]{figures/centroids_clustering_comunale.png} \\
    
    \bottomrule
    \end{tabular}
    \caption{Clustering results at municipality level. On the left the spatial distribution of the clusters. Municipalities depicted with the same color belong to the same cluster. On the right the relative centroids of the three identified clusters. The line colors correspond to the ones on the map.}
    \label{fig:clustering:comunale}
\end{figure}













==> old_tex/wai.tex <==
\section{Regression results}\label{sec:regression}

In this section, we present the results of the OLS regressions conducted as the third step of our methodological framework to evaluate if the location of a firm has an impact on its own WAI.
Regression results are summarized in Table \ref{tab:regression}.
The first two columns of Table \ref{tab:regression} report our baseline model (with the WAI as the dependent variable) in two different specifications: with SMEs and big firms and with micro, medium and big firms. 
The coefficient of the location in inner areas is significant and negative, as expected. The firm dimension is positive and significant for SMEs and big firms, while negative for micro firms (i.e., firms with less than 10 employees). This can be interpreted as a major attention paid to the digital tools by more structured firms to promote their business or to communicate more effectively with external stakeholders.
In the third column of Table \ref{tab:regression}, we analysed the WAI effects across different municipality categories, as described in Section \ref{sec:methodology}. As expected, the big urban poles variable has a significant and positive effect on the WAI, while in two out of three typologies of inner areas (namely ``intermediate'' and ``ultraperiphery'') the effect turns to be significant and negative.
Moreover, the fourth column of Table \ref{tab:regression} highlights that the north dummy (defined according to the location of NUTS-2 dummy)  has a positive and significant effect of the digital footprint measured through the WAI. Conversely, firms located in the south have a significanlty lower WAI. 
In all the regression tests, we can see that the same results concerning the sector of activity of the firm: manufacturing (code ``C''), wholesale and retail trade (code ``G''), Information and Communication (code ``J''), Professional, Scientific and Technical Activities (code ``M''), Financial and insurance activities (code ``K'') and Real estate activities (code ``L'') register a positive and significant effect, while Agriculture (code ``A''), Construction (code ``F''), Transportation and Storage (code ``H''), Accommodation and Food Service Activities (code ``I'') do not show any effect. The higher coefficients are in the Information and Communication (code ``J'') and Professional, Scientific and Technical Activities (code ``M'') sectors.
Once again, this validates our methodological framework, which is able to measure and spot the digital divide at different geographical scales, using the firms' homepages as a proxy of their digital culture.

\leo{à}
% città).




% \begin{table}[ht!]
% \centering
% \begin{tabular}{|l|l|l|} 
% \hline
% Features & Interactions  & Reference \\ 
% \hline
% Small Medium Big Aree Interne &  & \ref{tab:regression1}   \\ 
% \hline
% Micro Medium Big Aree Interne &  & \ref{tab:regression2}\\ 
% \hline
% Small Medium Big - Classificazione comuni &  & \ref{tab:regression3}   \\ 
% \hline
% % Small Medium Big Aree Interne &  Dimension:Macro sector & \ref{tab:regression1:interaction1}\\ 
% % \hline
% Small Medium Big Aree Interne & Dimension:Aree interne & \ref{tab:regression1:interaction2}\\ 
% \hline
% % Micro Medium Big Aree Interne & Dimension:Macro sector  & \ref{tab:regression2:interaction1}\\ 
% % \hline
% Micro Medium Big Aree Interne &  Dimension:Aree interne & \ref{tab:regression2:interaction2}\\ 
% \hline
% % Small Medium Big - Classificazione comuni & Dimension:Macro sector & \ref{tab:regression3:interaction1}\\ 
% % \hline
% Small Medium Big - Classificazione comuni & Dimension:Classificazione comuni  & \ref{tab:regression3:interaction2}   \\ 
% \hline
% \end{tabular}
% \caption{Summary of the regressions, with list of the features, and the relative tested interactions, if any.}
% \label{'tab:regression_summary'}
% \end{table}

\begin{table}[ht!]
\centering
\scriptsize
\begin{adjustbox}{max width=1.\textwidth,center}
\begin{tabular}{llllllllllll}
\toprule
{} &                    index &                unique\_links\_in &               unique\_links\_out &                 best-practices &                      instagram &                       linkedin &                       facebook &                      years\_old &            security\_header\_int &                   request\_time &                     length\_url \\
\midrule
0  &                    const &   \makecell{ 0.005*** \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} &   \makecell{ 0.771*** \\(0.002)} &  \makecell{ -0.965*** \\(0.027)} &  \makecell{ -1.810*** \\(0.032)} &   \makecell{ 0.376*** \\(0.022)} &   \makecell{ 0.406*** \\(0.003)} &   \makecell{ 0.415*** \\(0.001)} &   \makecell{ 0.010*** \\(0.000)} &   \makecell{ 0.143*** \\(0.000)} \\
1  &                    micro &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.000*** \\(0.000)} &  \makecell{ -0.005*** \\(0.001)} &  \makecell{ -0.236*** \\(0.013)} &  \makecell{ -0.576*** \\(0.016)} &  \makecell{ -0.136*** \\(0.011)} &  \makecell{ -0.093*** \\(0.002)} &   \makecell{ 0.012*** \\(0.001)} &   \makecell{ 0.001*** \\(0.000)} &   \makecell{ 0.002*** \\(0.000)} \\
2  &                   medium &   \makecell{ 0.002*** \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} &   \makecell{ 0.006*** \\(0.001)} &   \makecell{ 0.322*** \\(0.023)} &   \makecell{ 0.654*** \\(0.023)} &   \makecell{ 0.196*** \\(0.020)} &   \makecell{ 0.074*** \\(0.003)} &  \makecell{ -0.013*** \\(0.001)} &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.002*** \\(0.000)} \\
3  &                      big &   \makecell{ 0.005*** \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} &      \makecell{ 0.003 \\(0.003)} &   \makecell{ 0.505*** \\(0.042)} &   \makecell{ 1.113*** \\(0.040)} &   \makecell{ 0.339*** \\(0.038)} &   \makecell{ 0.109*** \\(0.005)} &  \makecell{ -0.029*** \\(0.002)} &     \makecell{ -0.001 \\(0.000)} &   \makecell{ -0.002** \\(0.001)} \\
4  &                        A &   \makecell{ -0.001** \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &      \makecell{ 0.001 \\(0.003)} &   \makecell{ 0.694*** \\(0.049)} &  \makecell{ -0.575*** \\(0.090)} &   \makecell{ 0.260*** \\(0.047)} &   \makecell{ 0.031*** \\(0.007)} &    \makecell{ -0.007* \\(0.003)} &     \makecell{ -0.000 \\(0.000)} &   \makecell{ -0.003** \\(0.001)} \\
5  &                        C &  \makecell{ -0.000*** \\(0.000)} &   \makecell{ -0.000** \\(0.000)} &     \makecell{ -0.001 \\(0.001)} &  \makecell{ -0.134*** \\(0.020)} &   \makecell{ 0.272*** \\(0.023)} &  \makecell{ -0.494*** \\(0.016)} &   \makecell{ 0.099*** \\(0.002)} &    \makecell{ -0.002* \\(0.001)} &   \makecell{ -0.000** \\(0.000)} &  \makecell{ -0.015*** \\(0.000)} \\
6  &                        G &   \makecell{ 0.003*** \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} &  \makecell{ -0.005*** \\(0.001)} &   \makecell{ 0.300*** \\(0.019)} &     \makecell{ -0.002 \\(0.024)} &     \makecell{ 0.033* \\(0.016)} &   \makecell{ 0.061*** \\(0.002)} &      \makecell{ 0.001 \\(0.001)} &   \makecell{ 0.001*** \\(0.000)} &  \makecell{ -0.010*** \\(0.000)} \\
7  &                        F &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.000*** \\(0.000)} &     \makecell{ -0.002 \\(0.002)} &  \makecell{ -0.804*** \\(0.031)} &  \makecell{ -0.194*** \\(0.033)} &  \makecell{ -0.653*** \\(0.022)} &  \makecell{ -0.012*** \\(0.003)} &   \makecell{ 0.010*** \\(0.001)} &   \makecell{ 0.001*** \\(0.000)} &  \makecell{ -0.004*** \\(0.000)} \\
8  &                        H &  \makecell{ -0.002*** \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &  \makecell{ -0.009*** \\(0.002)} &  \makecell{ -0.763*** \\(0.044)} &  \makecell{ -0.287*** \\(0.046)} &  \makecell{ -0.735*** \\(0.031)} &   \makecell{ 0.022*** \\(0.004)} &   \makecell{ 0.007*** \\(0.002)} &      \makecell{ 0.000 \\(0.000)} &  \makecell{ -0.003*** \\(0.001)} \\
9  &                        I &  \makecell{ -0.001*** \\(0.000)} &      \makecell{ 0.000 \\(0.000)} &  \makecell{ -0.015*** \\(0.002)} &   \makecell{ 0.904*** \\(0.024)} &  \makecell{ -1.411*** \\(0.052)} &   \makecell{ 0.741*** \\(0.023)} &   \makecell{ 0.045*** \\(0.003)} &     \makecell{ -0.002 \\(0.001)} &  \makecell{ -0.001*** \\(0.000)} &   \makecell{ 0.009*** \\(0.001)} \\
10 &                        J &   \makecell{ 0.001*** \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} &    \makecell{ 0.005** \\(0.002)} &  \makecell{ -0.262*** \\(0.029)} &   \makecell{ 1.275*** \\(0.028)} &  \makecell{ -0.133*** \\(0.023)} &   \makecell{ 0.070*** \\(0.003)} &  \makecell{ -0.019*** \\(0.001)} &  \makecell{ -0.002*** \\(0.000)} &  \makecell{ -0.027*** \\(0.001)} \\
11 &                        M &     \makecell{ -0.000 \\(0.000)} &      \makecell{ 0.000 \\(0.000)} &   \makecell{ 0.008*** \\(0.002)} &  \makecell{ -0.212*** \\(0.027)} &   \makecell{ 1.137*** \\(0.027)} &  \makecell{ -0.385*** \\(0.022)} &   \makecell{ 0.039*** \\(0.003)} &  \makecell{ -0.014*** \\(0.001)} &  \makecell{ -0.002*** \\(0.000)} &  \makecell{ -0.018*** \\(0.000)} \\
12 &                        K &    \makecell{ -0.001* \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &      \makecell{ 0.003 \\(0.004)} &  \makecell{ -0.982*** \\(0.080)} &   \makecell{ 0.723*** \\(0.059)} &  \makecell{ -0.709*** \\(0.051)} &     \makecell{ 0.017* \\(0.007)} &  \makecell{ -0.017*** \\(0.003)} &  \makecell{ -0.003*** \\(0.000)} &  \makecell{ -0.009*** \\(0.001)} \\
13 &                        L &      \makecell{ 0.001 \\(0.000)} &     \makecell{ 0.000* \\(0.000)} &  \makecell{ -0.011*** \\(0.003)} &   \makecell{ 0.168*** \\(0.043)} &   \makecell{ 0.263*** \\(0.052)} &      \makecell{ 0.036 \\(0.036)} &   \makecell{ 0.084*** \\(0.005)} &     \makecell{ -0.002 \\(0.002)} &     \makecell{ -0.001 \\(0.000)} &      \makecell{ 0.001 \\(0.001)} \\
14 &                   INPOLO &   \makecell{ 0.000*** \\(0.000)} &    \makecell{ 0.000** \\(0.000)} &      \makecell{ 0.001 \\(0.001)} &   \makecell{ 0.130*** \\(0.013)} &   \makecell{ 0.170*** \\(0.015)} &   \makecell{ 0.052*** \\(0.011)} &      \makecell{ 0.003 \\(0.002)} &     \makecell{ -0.002 \\(0.001)} &     \makecell{ -0.000 \\(0.000)} &  \makecell{ -0.002*** \\(0.000)} \\
15 &                    North &      \makecell{ 0.000 \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &   \makecell{ 0.011*** \\(0.001)} &  \makecell{ -0.102*** \\(0.015)} &   \makecell{ 0.288*** \\(0.018)} &  \makecell{ -0.201*** \\(0.012)} &   \makecell{ 0.019*** \\(0.002)} &  \makecell{ -0.008*** \\(0.001)} &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.005*** \\(0.000)} \\
16 &                    South &   \makecell{ 0.000*** \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &  \makecell{ -0.008*** \\(0.001)} &   \makecell{ 0.067*** \\(0.018)} &  \makecell{ -0.109*** \\(0.023)} &   \makecell{ 0.162*** \\(0.015)} &  \makecell{ -0.045*** \\(0.002)} &   \makecell{ 0.014*** \\(0.001)} &   \makecell{ 0.002*** \\(0.000)} &    \makecell{ 0.001** \\(0.000)} \\
17 &  anni\_dalla\_costituzione &  \makecell{ -0.000*** \\(0.000)} &      \makecell{ 0.000 \\(0.000)} &  \makecell{ -0.000*** \\(0.000)} &  \makecell{ -0.013*** \\(0.000)} &  \makecell{ -0.009*** \\(0.000)} &  \makecell{ -0.010*** \\(0.000)} &                            NaN &    \makecell{ 0.000** \\(0.000)} &     \makecell{ -0.000 \\(0.000)} &   \makecell{ 0.000*** \\(0.000)} \\
18 &                Wide\_band &    \makecell{ 0.000** \\(0.000)} &      \makecell{ 0.000 \\(0.000)} &      \makecell{ 0.001 \\(0.001)} &     \makecell{ 0.043* \\(0.017)} &   \makecell{ 0.131*** \\(0.020)} &      \makecell{ 0.015 \\(0.014)} &    \makecell{ -0.004* \\(0.002)} &      \makecell{ 0.002 \\(0.001)} &      \makecell{ 0.000 \\(0.000)} &     \makecell{ -0.000 \\(0.000)} \\
19 &               R-squared: &                          0.028 &                          0.002 &                          0.005 &                            NaN &                            NaN &                            NaN &                          0.071 &                          0.013 &                          0.009 &                          0.041 \\
20 &          Adj. R-squared: &                          0.027 &                          0.002 &                          0.005 &                            NaN &                            NaN &                            NaN &                          0.071 &                          0.013 &                          0.009 &                          0.041 \\
\bottomrule
\end{tabular}


\end{adjustbox}
\caption{\label{tab:regression_features} OLS regression results. The dependent variable is the WAI index of firms in all regressions.}
\end{table}


\begin{table}[ht!]
\centering
\scriptsize
\begin{adjustbox}{max width=1.\textwidth,center}

\begin{tabular}{lllllll}
\toprule
{} &                    index &         stakekholder\_eng\_index &   technical\_capabilities\_index &          digital\_culture\_index &    internal\_organization\_index &                  new\_wai\_index \\
\midrule
0  &                    const &   \makecell{ 0.827*** \\(0.006)} &   \makecell{ 2.346*** \\(0.002)} &   \makecell{ 0.252*** \\(0.003)} &   \makecell{ 0.862*** \\(0.001)} &   \makecell{ 1.672*** \\(0.003)} \\
1  &                    micro &  \makecell{ -0.076*** \\(0.003)} &  \makecell{ -0.018*** \\(0.001)} &  \makecell{ -0.049*** \\(0.001)} &  \makecell{ -0.003*** \\(0.000)} &  \makecell{ -0.075*** \\(0.002)} \\
2  &                   medium &   \makecell{ 0.119*** \\(0.005)} &   \makecell{ 0.020*** \\(0.002)} &   \makecell{ 0.040*** \\(0.003)} &   \makecell{ 0.004*** \\(0.000)} &   \makecell{ 0.079*** \\(0.003)} \\
3  &                      big &   \makecell{ 0.221*** \\(0.010)} &   \makecell{ 0.033*** \\(0.004)} &   \makecell{ 0.058*** \\(0.005)} &   \makecell{ 0.007*** \\(0.001)} &   \makecell{ 0.128*** \\(0.006)} \\
4  &                        A &     \makecell{ 0.029* \\(0.012)} &      \makecell{ 0.009 \\(0.005)} &  \makecell{ -0.028*** \\(0.006)} &     \makecell{ 0.003* \\(0.001)} &    \makecell{ -0.017* \\(0.007)} \\
5  &                        C &   \makecell{ 0.132*** \\(0.004)} &      \makecell{ 0.002 \\(0.002)} &   \makecell{ 0.064*** \\(0.002)} &   \makecell{ 0.015*** \\(0.000)} &   \makecell{ 0.105*** \\(0.003)} \\
6  &                        G &   \makecell{ 0.047*** \\(0.004)} &  \makecell{ -0.008*** \\(0.002)} &   \makecell{ 0.037*** \\(0.002)} &   \makecell{ 0.013*** \\(0.000)} &   \makecell{ 0.053*** \\(0.003)} \\
7  &                        F &   \makecell{ 0.033*** \\(0.005)} &  \makecell{ -0.014*** \\(0.002)} &  \makecell{ -0.022*** \\(0.003)} &   \makecell{ 0.002*** \\(0.000)} &  \makecell{ -0.018*** \\(0.003)} \\
8  &                        H &   \makecell{ 0.039*** \\(0.008)} &  \makecell{ -0.017*** \\(0.003)} &     \makecell{ -0.001 \\(0.004)} &      \makecell{ 0.001 \\(0.001)} &      \makecell{ 0.004 \\(0.005)} \\
9  &                        I &  \makecell{ -0.074*** \\(0.006)} &  \makecell{ -0.011*** \\(0.002)} &   \makecell{ 0.051*** \\(0.003)} &  \makecell{ -0.009*** \\(0.001)} &   \makecell{ 0.024*** \\(0.004)} \\
10 &                        J &   \makecell{ 0.201*** \\(0.006)} &   \makecell{ 0.026*** \\(0.002)} &   \makecell{ 0.079*** \\(0.003)} &   \makecell{ 0.028*** \\(0.001)} &   \makecell{ 0.152*** \\(0.004)} \\
11 &                        M &   \makecell{ 0.238*** \\(0.006)} &   \makecell{ 0.023*** \\(0.002)} &   \makecell{ 0.048*** \\(0.003)} &   \makecell{ 0.018*** \\(0.001)} &   \makecell{ 0.124*** \\(0.003)} \\
12 &                        K &   \makecell{ 0.149*** \\(0.013)} &   \makecell{ 0.023*** \\(0.005)} &      \makecell{ 0.011 \\(0.007)} &   \makecell{ 0.008*** \\(0.001)} &   \makecell{ 0.060*** \\(0.008)} \\
13 &                        L &   \makecell{ 0.050*** \\(0.009)} &    \makecell{ -0.008* \\(0.004)} &   \makecell{ 0.048*** \\(0.005)} &     \makecell{ -0.000 \\(0.001)} &   \makecell{ 0.058*** \\(0.006)} \\
14 &                   INPOLO &   \makecell{ 0.030*** \\(0.003)} &    \makecell{ 0.003** \\(0.001)} &    \makecell{ 0.004** \\(0.001)} &   \makecell{ 0.003*** \\(0.000)} &   \makecell{ 0.014*** \\(0.002)} \\
15 &                    North &   \makecell{ 0.067*** \\(0.003)} &   \makecell{ 0.020*** \\(0.001)} &   \makecell{ 0.007*** \\(0.002)} &   \makecell{ 0.005*** \\(0.000)} &   \makecell{ 0.033*** \\(0.002)} \\
16 &                    South &  \makecell{ -0.038*** \\(0.004)} &  \makecell{ -0.024*** \\(0.002)} &  \makecell{ -0.030*** \\(0.002)} &    \makecell{ -0.001* \\(0.000)} &  \makecell{ -0.048*** \\(0.002)} \\
17 &  anni\_dalla\_costituzione &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.000*** \\(0.000)} &   \makecell{ 0.007*** \\(0.000)} &  \makecell{ -0.000*** \\(0.000)} &   \makecell{ 0.006*** \\(0.000)} \\
18 &                Wide\_band &   \makecell{ 0.018*** \\(0.004)} &     \makecell{ -0.001 \\(0.001)} &     \makecell{ -0.001 \\(0.002)} &      \makecell{ 0.000 \\(0.000)} &      \makecell{ 0.003 \\(0.002)} \\
19 &               R-squared: &                          0.049 &                          0.014 &                           0.17 &                          0.043 &                          0.168 \\
20 &          Adj. R-squared: &                          0.048 &                          0.014 &                           0.17 &                          0.043 &                          0.168 \\
\bottomrule
\end{tabular}

\end{adjustbox}
\caption{\label{tab:regressionnew_wai} OLS regression results. The dependent variable is the WAI index of firms in all regressions.}
\end{table}


\begin{table}[ht!]
\centering
\scriptsize
\begin{adjustbox}{max width=1.\textwidth,center}

\begin{tabular}{lllllll}
\toprule
{} &                    index &             navigability\_index &            accessibility\_index &                    speed\_index &        digital\_culture\_2\_index &                        old\_wai \\
\midrule
0  &                    const &   \makecell{ 0.777*** \\(0.002)} &   \makecell{ 1.683*** \\(0.006)} &   \makecell{ 0.990*** \\(0.000)} &   \makecell{ 0.837*** \\(0.003)} &   \makecell{ 2.088*** \\(0.002)} \\
1  &                    micro &  \makecell{ -0.006*** \\(0.001)} &  \makecell{ -0.077*** \\(0.003)} &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.061*** \\(0.002)} &  \makecell{ -0.053*** \\(0.001)} \\
2  &                   medium &   \makecell{ 0.008*** \\(0.001)} &   \makecell{ 0.121*** \\(0.005)} &   \makecell{ 0.001*** \\(0.000)} &   \makecell{ 0.054*** \\(0.003)} &   \makecell{ 0.060*** \\(0.002)} \\
3  &                      big &    \makecell{ 0.008** \\(0.003)} &   \makecell{ 0.223*** \\(0.010)} &      \makecell{ 0.001 \\(0.000)} &   \makecell{ 0.087*** \\(0.006)} &   \makecell{ 0.103*** \\(0.004)} \\
4  &                        A &      \makecell{ 0.000 \\(0.003)} &    \makecell{ 0.033** \\(0.012)} &      \makecell{ 0.000 \\(0.000)} &   \makecell{ -0.021** \\(0.007)} &     \makecell{ -0.002 \\(0.005)} \\
5  &                        C &     \makecell{ -0.001 \\(0.001)} &   \makecell{ 0.147*** \\(0.004)} &    \makecell{ 0.000** \\(0.000)} &   \makecell{ 0.066*** \\(0.002)} &   \makecell{ 0.070*** \\(0.002)} \\
6  &                        G &    \makecell{ -0.003* \\(0.001)} &   \makecell{ 0.057*** \\(0.004)} &  \makecell{ -0.001*** \\(0.000)} &   \makecell{ 0.036*** \\(0.002)} &   \makecell{ 0.030*** \\(0.002)} \\
7  &                        F &    \makecell{ -0.004* \\(0.002)} &   \makecell{ 0.037*** \\(0.005)} &  \makecell{ -0.001*** \\(0.000)} &  \makecell{ -0.033*** \\(0.003)} &  \makecell{ -0.009*** \\(0.002)} \\
8  &                        H &  \makecell{ -0.011*** \\(0.002)} &   \makecell{ 0.042*** \\(0.008)} &     \makecell{ -0.000 \\(0.000)} &     \makecell{ -0.008 \\(0.004)} &      \makecell{ 0.002 \\(0.003)} \\
9  &                        I &  \makecell{ -0.015*** \\(0.002)} &  \makecell{ -0.083*** \\(0.006)} &   \makecell{ 0.001*** \\(0.000)} &   \makecell{ 0.053*** \\(0.003)} &      \makecell{ 0.002 \\(0.002)} \\
10 &                        J &   \makecell{ 0.006*** \\(0.002)} &   \makecell{ 0.227*** \\(0.006)} &   \makecell{ 0.002*** \\(0.000)} &   \makecell{ 0.098*** \\(0.003)} &   \makecell{ 0.110*** \\(0.002)} \\
11 &                        M &   \makecell{ 0.008*** \\(0.002)} &   \makecell{ 0.256*** \\(0.006)} &   \makecell{ 0.002*** \\(0.000)} &   \makecell{ 0.062*** \\(0.003)} &   \makecell{ 0.099*** \\(0.002)} \\
12 &                        K &      \makecell{ 0.003 \\(0.004)} &   \makecell{ 0.158*** \\(0.013)} &   \makecell{ 0.003*** \\(0.000)} &   \makecell{ 0.028*** \\(0.007)} &   \makecell{ 0.057*** \\(0.005)} \\
13 &                        L &  \makecell{ -0.010*** \\(0.003)} &   \makecell{ 0.049*** \\(0.009)} &      \makecell{ 0.001 \\(0.000)} &   \makecell{ 0.050*** \\(0.005)} &   \makecell{ 0.035*** \\(0.004)} \\
14 &                   INPOLO &      \makecell{ 0.001 \\(0.001)} &   \makecell{ 0.033*** \\(0.003)} &      \makecell{ 0.000 \\(0.000)} &   \makecell{ 0.006*** \\(0.002)} &   \makecell{ 0.012*** \\(0.001)} \\
15 &                    North &   \makecell{ 0.011*** \\(0.001)} &   \makecell{ 0.072*** \\(0.003)} &   \makecell{ 0.001*** \\(0.000)} &   \makecell{ 0.015*** \\(0.002)} &   \makecell{ 0.030*** \\(0.001)} \\
16 &                    South &  \makecell{ -0.008*** \\(0.001)} &  \makecell{ -0.039*** \\(0.004)} &  \makecell{ -0.002*** \\(0.000)} &  \makecell{ -0.044*** \\(0.002)} &  \makecell{ -0.036*** \\(0.002)} \\
17 &  anni\_dalla\_costituzione &  \makecell{ -0.000*** \\(0.000)} &  \makecell{ -0.001*** \\(0.000)} &      \makecell{ 0.000 \\(0.000)} &   \makecell{ 0.007*** \\(0.000)} &   \makecell{ 0.003*** \\(0.000)} \\
18 &                Wide\_band &      \makecell{ 0.001 \\(0.001)} &   \makecell{ 0.019*** \\(0.004)} &     \makecell{ -0.000 \\(0.000)} &     \makecell{ -0.003 \\(0.002)} &     \makecell{ 0.004* \\(0.001)} \\
19 &               R-squared: &                          0.005 &                          0.054 &                          0.009 &                          0.154 &                          0.136 \\
20 &          Adj. R-squared: &                          0.005 &                          0.054 &                          0.009 &                          0.154 &                          0.136 \\
\bottomrule
\end{tabular}


\end{adjustbox}
\caption{\label{tab:regression_old_wai} OLS regression results. The dependent variable is the WAI index of firms in all regressions.}
\end{table}



\begin{table}[ht!]
\centering
\scriptsize
\begin{adjustbox}{max width=1.\textwidth,center}
\begin{tabular}{lll}
\toprule
{} &                    index &                     summed\_wai \\
\midrule
0  &                    const &   \makecell{ 2.601*** \\(0.011)} \\
1  &                    micro &  \makecell{ -0.178*** \\(0.006)} \\
2  &                   medium &   \makecell{ 0.244*** \\(0.010)} \\
3  &                      big &   \makecell{ 0.416*** \\(0.019)} \\
4  &                        A &   \makecell{ 0.115*** \\(0.023)} \\
5  &                        C &  \makecell{ -0.064*** \\(0.008)} \\
6  &                        G &   \makecell{ 0.088*** \\(0.008)} \\
7  &                        F &  \makecell{ -0.299*** \\(0.011)} \\
8  &                        H &  \makecell{ -0.321*** \\(0.015)} \\
9  &                        I &   \makecell{ 0.311*** \\(0.011)} \\
10 &                        J &   \makecell{ 0.172*** \\(0.011)} \\
11 &                        M &   \makecell{ 0.071*** \\(0.011)} \\
12 &                        K &  \makecell{ -0.205*** \\(0.024)} \\
13 &                        L &   \makecell{ 0.101*** \\(0.018)} \\
14 &                   INPOLO &   \makecell{ 0.055*** \\(0.005)} \\
15 &                    North &  \makecell{ -0.026*** \\(0.006)} \\
16 &                    South &     \makecell{ 0.019* \\(0.008)} \\
17 &  anni\_dalla\_costituzione &   \makecell{ 0.001*** \\(0.000)} \\
18 &                Wide\_band &   \makecell{ 0.027*** \\(0.007)} \\
0  &               R-squared: &                          0.038 \\
1  &          Adj. R-squared: &                          0.038 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{tab:regression_summed} OLS regression results. The dependent variable is the WAI index of firms in all regressions.}
\end{table}



\begin{table}[ht!]
\centering
\scriptsize
\begin{adjustbox}{max width=1.\textwidth,center}
\begin{tabular}{lllll}
\hline
\textbf{Variable} & \textbf{Model 1} & \textbf{Model 2} & \textbf{Model 3} & \textbf{Model 4} \\
\midrule
\textbf{Micro firm}                &                         & -0.0478***               &                &         \\
\textbf{}                     &                         & (0.001)                  &               &          \\
\textbf{Small firm}                &    0.0478***                     &                          & 0.0479***      &       0.0480***           \\
\textbf{}                     &     (0.001)                    &                          &   (0.001)        &      (0.001)           \\
\textbf{Medium firm}               &       0.0980***                  &    0.0502***                      &             0.0979***     & 0.0985***       \\
\textbf{}                     &          (0.002)               &       (0.002)                    &         (0.001)      & (0.002)         \\
\textbf{Large firm}                  &         0.1351***                &    0.0873***                      &          0.1345***    &  0.1356***         \\
\textbf{}                     &            (0.004)             &   (0.004)                        &        (0.004)      &   (0.004)        \\
\textbf{Firm age}            &  0.0031***                       &     0.0031***                     &   0.0031***  &     0.0031***                \\
\textbf{}                     &    (4.4e-05)                     &       (4.4e-05)                   &      (4.4e-05)   &    (4.4e-05)              \\
\textbf{Agriculture - A}                    &            0.0038             &           0.0038               &       0.0052    &   0.0036          \\
\textbf{}                     &              (0.006)           &      (0.006)                    &    (0.006)      &    (0.006)           \\
\textbf{Manufacturing - C}                    &           0.0716***              &        0.0716***                  &          0.0737***        &    0.0724***        \\
\textbf{}                     &       (0.002)                  &      (0.002)                    &       (0.002)      &    (0.002)          \\
\textbf{Wholesale and retail trade - G}                    &    0.0207***                     & 0.0207***                            &    0.0215***     &     0.0212***              \\
\textbf{}                     &          (0.002)              &     (0.002)                      &        (0.002)       &   (0.002)       \\
\textbf{Construction - F}                    &         -0.0034                &       -0.0034                    &    -0.0022  &        -0.0031            \\
\textbf{}                     &        (0.003)                 &      (0.003)                      &           (0.003)    &  (0.269)         \\
\textbf{Transportation and Storage - H}                    &   0.0060                       & 0.0060                         &     0.0064   &         0.0059          \\
\textbf{}                     &          (0.004)               &      (0.004)                     &                (0.004)      & (0.132)    \\
\textbf{Accommodation and Food Service Activities - I}                    &   0.0035                      &     0.0035                     &     0.0036        &     0.0042        \\
\textbf{}                     &     (0.003)                    &   (0.003)                        &          (0.003)       &    (0.003)     \\
\textbf{Information and Communication - J}                    &   0.1096***                      &  0.1096***                          &    0.1089***       &    0.1100***          \\
\textbf{}                     &     (0.003)                    &       (0.003)                    &   (0.003)      &   (0.003)              \\
\textbf{Professional, Scientific and Technical Activities - M}                    &   0.1021***                     &     0.1021***                     &      0.1014***          &      0.1027***    \\
\textbf{}                     &      (0.003)                   &     (0.003)                      &    (0.003)           &    (0.003)      \\
\textbf{Financial and insurance activities - K}                    &    0.0563***                     &            0.0563***                 &    0.0550***     &   0.0565***             \\
\textbf{}                     &       (0.007)                 &           (0.007)                  &  (0.007)    &        (0.007)               \\
\textbf{Real estate activities - L}                    &   0.0361***                      &   0.0361***                        &   0.0360***        &   0.0375***           \\
\textbf{}                     &       (0.005)                  &    (0.005)                       &     (0.005)    &  (0.005)                 \\
\textbf{Inner Areas}         &     -0.0125***                    &        -0.0125***                  &            &   -0.0137***          \\
\textbf{}                     &     (0.002)                    &         (0.002)                 &            &     (0.002)        \\
\textbf{A-"Urban pole"}               &                         &                          &     0.0084***       &             \\
\textbf{}                     &                         &                          &     (0.001)        &            \\
\textbf{B-"Suburban area"} &                         &                          &   -0.0009        &              \\
\textbf{}                     &                         &                          &        (0.003)     &            \\
\textbf{D-"Intermediate"}         &                         &                          &  -0.00099***    &                   \\
\textbf{}                     &                         &                          &        (0.002)    &             \\
\textbf{E-"Periphery"}         &                         &                          &    0.0005      &               \\
\textbf{}                     &                         &                          &     (0.004)      &               \\
\textbf{F-"Ultraperiphery"}    &                         &                          &         -0.0260**        &        \\
\textbf{}                     &                         &                          &      (0.008)                    \\
\textbf{North}            &                        &                          &     &       0.0314***             \\
\textbf{}                     &                      &                &        &          (0.002)         \\
\textbf{South}            &                        &                          &   &       -0.0404***             \\
\textbf{}                     &                     &                      &        &        (0.002)          \\
\textbf{NUT-2 Dummy}          &        YES                 &         YES                 &  YES          & NO             \\

\textbf{Constant}             &    2.5867***                       &   2.6345***                       &       2.5818***      &   2.5820***         \\
\textbf{}                     &   (0.014)                          &   (0.014)                        &     (0.014)       &     (0.002)        \\
\midrule
\textbf{N. of Observations}   &          148\,797         &    148\,797                &          148\,797  &  148\,797    \\
\textbf{R-squared:}   &          0.123         &    0.123                &          0.123   &   0.121  \\
\textbf{AIC}   &          -4719         &    -4719                &          -4759     &  -4452  \\
\textbf{BIC}   &          -4362         &    -4362                &          -4362   &   -4273   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{tab:regression} OLS regression results. The dependent variable is the WAI index of firms in all regressions.}
\end{table}



\section{Web Assessment Index}\label{sec:wai}

Analysing the quality of websites is a complex task for the presence of several unstructured information that need to be framed into logical theoretical schemes to understand their potential economic value. The literature that deals with website analysis has underlined how the quality of a website is a multifaceted concept, which can be observed by several points of view: technical, social, legal and purely economic \citep{KrolandZdonek2020}. Its high degree of customisation makes difficult establishing objective criteria of evaluation. Within this literature, \cite{Mateosetal2001} provide one of the first web assessment tools tested on universities websites. They consider four dimensions of analysis: site content, speed, accessibility and navigability. While the first two are quite straightforward, the last two need to be explicitly framed. As underlined also by \cite{Vaughan2004} accessibility has been proxied respectively by search engines indexes and popularity (number of external links can imply more traffic). Navigability has been mainly measured as the number of steps (clicks) to access relevant information for the user. Other measures have been introduced as usability, which can be seen as an extension of navigability, more oriented to convenience of users to navigate the website for several reasons, as easiness, responsivity, and aesthetic reasons, which have become crucial especially in the last years to retain and acquire users \citep{Mateosetal2001, DickingerandStangl2013, KrolandZdonek2020}. 
More recently, multimedia elements (e.g. images, videos and sounds) have skyrocketed as means of communication thanks to the introduction of new technological enablers (e.g. high speed broadband), as well as website design becomes an important method to establish website quality \citep{RasmussenandThimm2015}. In addition, loading time has become another parameter to observe, considering also the myriad of legal and business services that have progressively emerged thanks to cloud computing. Notwithstanding, it is important to underline how the evaluation of websites should consider technological stack such as library and programming languages as more objective information (and thus less manipulable) in comparison to content and experience.

In our work, we aggregated the features presented in section 4 across four dimensions, as in the Web Assessment Index (WAI), developed by \cite{Mateosetal2001}, namely Accessibility, Navigability, Speed and Digital Culture. The latter substitutes the orginal dimension -- ``site content'' -- removed from the present analysis to rely on the more objective elements. Table \ref{tab:features} summarizes all the features extracted aggregated in four groups.

\begin{table}[ht!]
\centering
\begin{tabular}{|l|l|}
\hline
\textbf{Indicator}                          & \textbf{WAI Dimension}   \\
\hline
URL Lenght                         & \multirow{5}{*}{Accessibility}                 \\
SEO Performance                    &                 \\
Facebook                           &    \\
Instagram                          &                 \\
Linkedin                           &                 \\
\hline
Quality of internal links          & \multirow{3}{*}{Navigability}                \\
Quality of external links          &     \\
Quality of the technical framework &                 \\
\hline
Request access time                & Speed           \\
\hline
Web's site age                     & \multirow{2}{*}{Digital culture} \\
Security                           &                \\
\hline
\end{tabular}
\caption{\label{tab:features}Web Quality Index: indicators and dimensions. }
\end{table}

To build the WAI we normalise the variables with a $MinMax$ technique, inverting the scale of the values where necessary (the length of the URL, Facebook, request time, security header) for the purpose of interpretability. Then, we calculated the WAI as the weighted sum of each element as follows:
\begin{equation}
\label{eq:wai}
WAI = (accessibility/5) + (navigability/3)+ (speed)+ (digital\_culture/2)
\end{equation}


% \begin{table}[t!]
% \centering
% \begin{adjustbox}{width=1\textwidth}
% \begin{tabular}{ |l|l|l||l|} 
% \hline
% \textbf{Indicator} & \textbf{WAI dimension} \\
% \hline
% Length of the URL 
% SEO performance
% Facebook
% Instagram
% LinkedIn
% & Accessibility \\ 

% Quality of internal links
% Quality of external links
% Quality of the technical frameworks
% & Navigability \\ 

% Request access time
% & Speed \\ 

% Website's age
% Website security
% & Digital Culture \\ 
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{\label{tab:features}Web Quality Index: indicators and dimensions. }
% \end{table}
% \todo[Fabio]{migliorare leggibilità tabella separando meglio ogni indicatore}


Figure \ref{fig:wai} maps the WAI across Italian NUTS-3 regions and municipalities. The maps of the WAI distribution closely matches the result of the clustering exercise. The composition of orange group in figure \ref{fig:clustering:provinciale} changes with the WAI mapping, with some NUTS-3 regions located in the north-east part of the countries with similar values to central regions.

\begin{figure}[h!]
    \centering
    \begin{tabular}{ccc}
    \toprule
    \includegraphics[width=0.48\columnwidth]{figures/old_wai.png &
    \includegraphics[width=0.48\columnwidth]{figures/new_wai_index.png} \\
    \includegraphics[width=0.48\columnwidth]{figures/summed_wai.png} \\
    \bottomrule
    \end{tabular}
    \caption{The distribution of the Web Assessment Index (WAI) across Italian regions. On the left: the WAI distribution at NUTS3 level. On the right: the WAI distribution at municipality level. Municipality will less than 10 observations are not reported.}
    \label{fig:wai}
\end{figure}

% \todo[FABIO]{Inserire le MAPPE WAI per penetrazione di quartili per provincia. Credo sia importante per confermare quanto detto sopra. Se c'è tempo in appendice metterei anche le mappe delle 4 dimensioni del WAI}



